Twin-in-the-loop state estimation for vehicle dynamics control: theory and experiments

In vehicle dynamics control, many variables of interest cannot be directly measured, as sensors might be costly, fragile, or even not available. Therefore, real-time estimation techniques need to be used. The previous approach suffers from two main drawbacks: (i) the approximations due to model mismatch might jeopardize the performance of the final estimation-based control; (ii) each new estimator requires the calibration from scratch of a dedicated model. In this paper, we propose a twin-in-the-loop scheme, where the ad-hoc model is replaced by an accurate multibody simulator of the vehicle, typically available to vehicles manufacturers and suitable for the estimation of any onboard variable, coupled with a compensator within a closed-loop observer scheme. Given the black-box nature of the digital twin, a data-driven methodology for observer tuning is developed, based on Bayesian optimization. The effectiveness of the proposed estimation method for the estimation of vehicle states and forces, as compared to traditional model-based Kalman filtering, is experimentally shown on a dataset collected with a sports car.

==> old_stuff.tex <==
% \begin{itemize}
%  \item [.] Opening discussion about the actual automotive scenario and the main challenges in vehicle dynamics control. Focus about the state estimation problem, related to speed and side-slip and highlighting the importance of parameters and tire-road contact forces estimation inside this framework.\\
% Literature analysis about estimation for vehicle dynamic control systems (survey \cite{singh2018literature} and \cite{viehweger2020vehicle}) :
%  \begin{itemize}
    %  \item \textbf{Vehicle velocities}: \cite{chu2010vehicle} estimation of longitudinal and lateral velocities using a bicycle model with an EKF; longitudinal velocity with a kinematic model in \cite{tanelli2006longitudinal} and \cite{chu2011design}; estimation of the three-axis velocities with a kinematic approach \cite{oh2011design}. Moving horizon strategy in \cite{WANG_2004}.
    %  %
    %  \item \textbf{Side-slip}:\\
    %   kinematic based approaches in \cite{selmanaj2017vehicle}. \\
    %   \textit{Single Track model:}\cite{BAFFET20091255} employs an EKF appliied to a single track model as the second block of a modular observer. linear kalman filter on a single track model in \cite{Jiang_ITSC} in a  scheme made four modules; in \cite{ZhangICEMI} side-slip is estimated from tire-road contact forces using a single track model.
    %   \textit{Double track model:}
    %   \cite{DOUMIATI_ACC2010}: double track model with EKF; comparison between EKF and UKF in  \cite{DOUMIATI_IEEE_TM};
    %   \\
    %   the authors of \cite{breschi2020vehicle} proposes a LPV model to estimate side-slip via a kerner-based identification of a nonparametric model.
       %    
    %  \item \textbf{Vehicle and additional parameters:} Mass estimation via RLS algorithms \cite{FATHY_2008}, mass estimation and road slope \cite{VAHIDI_2005}; inertial parameters estimation \cite{rozyn2010method}.\\
    %
    %  \item \textbf{Tire-road forces}: \\
    %  \begin{enumerate}
    %      \item \textbf{Fx-Fy}\\
    %           \textit{Single Track model:}\cite{BAFFET20091255} employs SMO applied to a single track model to estimate front and rear forces (per axle) before estimating side-slip and cornering stiffness. \cite{WILKIN} uses an EKF to estimate total longitudinal and lateral forces (per axle).  \cite{Jiang_ITSC} employed an two different EKF to estimate longitudinal and lateral forces (per axle) based on the single track. in \cite{ZhangICEMI} a SMO approach is used to estimate the longitudinal and lateral forces (per axle). \cite{MSIRDI_VSD} enlarges the single track model with the relaxation dynamics in a SMO approach. \cite{HAMANN_IVS} extends the EKF to UKF still using a single track model.  \cite{HSIAO_2011} two step estimation of longitudinal (wheel equation) and lateral forces (single track) employing also friction ellipse. constraints.  \cite{rezaeian2014novel}  makes use also of a wheel dynamics model, with the single track, to robustly estimate longitudinal forces.
    %  \textit{Double track model:}
    %          \cite{DOUMIATI_ACC2010}: double track model with EKF to estimate forces at each wheel with vertical forces based split; \cite{DOUMIATI_IEEE_TM},\cite{DOUMIATI_ECC2009}: comparison between EKF and UKF with double track model and lateral tire model.\cite{ACARMAN}: forces estimation (lateral and longitudinal) with a double track model and SMO-like approach. \cite{SHRAIM_2007}: estimate longitudinal forces with SMO;
    %  \item \textbf{Fz}
    %         \cite{DOUMIATI_2008_IFAC}: linear quarter-car model based on Kalman Filter to estimate vertical forces,\cite{JIANG_2015}: more complex model accounting roll and pitch dynamics (quarters coupling).
    %  \end{enumerate}

     %
    %  \item \textbf{tire force measurements}: \cite{KRIER_2014} in-tire sensors to measure forces;\cite{BLASCO_2014} Design of Dynamo-metric Wheel Rim.
%  \end{itemize}
    % \begin{itemize}
        % \item [\&] \textbf{(COMPLEX model)} \cite{RayCST}: 9 dof model for forces and state estimation in simulation environment 
        % \item [\&] \textbf{(EKF-single track)}\cite{BAFFET20091255}: 2 blocks estimate on a single-track model(Front/Rear Forces-SMO and beta,C-EKF); \cite{BAFFET_IEEETM}: single track model plus simplified adaptive lateral tire force model (estimated friction), estimation of Forces (total Fx and F/R Fy) and vehicle state (beta) with EKF; \cite{WILKIN}: single track model with EKF only forces estimation; \cite{Jiang_ITSC}: fusion of four different observer to estimate longitudinal,lateral forces, beta and load transfer with a single track model.
        % \item [\&] \textbf{(SMO-single track)}\cite{ZhangICEMI}: tire forces, vehicle sideslip through a SMO approach employing a simple single-track model; \cite{MSIRDI_VSD} SMO to estimate forces employing single track plus relaxation dynamics.
        % \item [\&] \textbf{(UKF-single track)} \cite{HAMANN_IVS}: standard single track with extended force states employing UKF instead of EKF.
        % \item [\&] \textbf{(EKF/UKF - Double track)} \cite{BAFFET_VSD}: the authors of \cite{BAFFET20091255} employs a Double track model with the same EKF approch; \cite{DOUMIATI_ACC2010}: double track model with EKF to estimate forces at each wheel with vertical forces based split; \cite{DOUMIATI_IEEE_TM},\cite{DOUMIATI_ECC2009}: comparison between EKF and UKF with double track model and lateral tire model.
        %  \item [\&] \cite{JABALLAH_2014} SMO to estimate tire forces and ground slope on an agricultural vehicle; \cite{RABHI_2007} estimate friction and friction force with SMO and robust differentiator for angular acceleration.
        %  \item [\&] \cite{HSIAO_2011} two step estimation of longitudinal (wheel equation) and lateral forces (single track) employing also friction ellipse constraints.
        %  \item [\&] \cite{WANG_2004} Moving Horizon Strategy for vehicle speed and longitudinal friction force
        %  \item [\&] \textbf{Vertical Forces} \cite{DOUMIATI_2008_IFAC}: linear quarter-car model based on Kalman Filter to estimate vertical forces,\cite{JIANG_2015}: more complex model accounting roll and pitch dynamics (quarters coupling).
    % \end{itemize}
% \item [.] Main limitations of the available approaches:
%         \begin{itemize}
%         \item [-] simple models with intrinsic limited description capabilities, thus difficult to provide direct estimation of forces at each wheel for example.
%         \item [-] dedicated approach for each variable to be estimated (many models that must be continuously maintained).
%     \end{itemize}
%     \item [.] Introduction to what we propose: employment of a vehicle simulator in the observer-loop. Fig. \ref{fig:est_problem}; \textbf{reference to the implementation problem?} technological improvements expected in the next 3 (??) years pushed by autonomous driving requirements to motivate the approach usefulness. but also an important motivation is related to the necessity of car manufacturer to have a reliable and maintained simulator available for many development reasons, making feasible to employ this solution.
%     % \begin{figure}[h!]
%     % \centering
%     % \includegraphics[width=\columnwidth,trim={5.5cm 3cm 6cm 3cm},clip]{figures/general_estimation_problem.pdf}
%     % \caption{Simulator-based estimation framework: the synergy between the vehicle simulator and the closed-loop correction modules allows to estimate vehicle states and tire-road contact forces employing available online measurements.}
%     % \label{fig:est_problem}
%     % \end{figure}
%     \item [.] Innovative contributions:
%     \begin{itemize}
%         \item [+] quantum lip in the vehicle state estimation: unseen approach in literature in this field.
%         \item [+] Potentially high performance due to the high fidelity model
%         \item [+] Complex Models allows to observe "fine" vehicle variables, not present in simple models.
%         \item [+] Unique framework for estimation.
%     \end{itemize}
%    
%      \item [.] Main challenges addressed and proposed solutions:
%      \begin{itemize}
%          \item [?] Possible high dimensional problem given the amount of states and output variables $->$ "simple" linear structure (kalman-filter or luenberger like) $->$ sparsity enforcement.
%          \item [?] closed-loop correction tuning: unavailable mathematical system model $->$ necessity of a model-free approach based on data $->$ simulation-error-minimization approach based on bayesian optimization, see \cite{FRAZIER_2018} and \cite{SHAHRIARI_2015}. \textbf{Add Literature about bay opt application in vehicle dynamics and observer tuning, if any.}
%      \end{itemize}
% \end{itemize}
